Thompson Sampling in Switching Environments with Bayesian Online Change Point Detection

Thompson Sampling has recently been shown to be optimal in the Bernoulli Multi-Armed Bandit setting[Kaufmann et al., 2012]. This bandit problem assumes stationary distributions for the rewards. It is often unrealistic to model the real world as a stationary distribution. In this paper we derive and evaluate algorithms using Thompson Sampling for a Switching Multi-Armed Bandit Problem. We propose a Thompson Sampling strategy equipped with a Bayesian change point mechanism to tackle this problem. We develop algorithms for a variety of cases with constant switching rate: when switching occurs all arms change (Global Switching), switching occurs independently for each arm (Per-Arm Switching), when the switching rate is known and when it must be inferred from data. This leads to a family of algorithms we collectively term Change-Point Thompson Sampling (CTS). We show empirical results of the algorithm in 4 artificial environments, and 2 derived from real world data; news click-through[Yahoo!, 2011] and foreign exchange data[Dukascopy, 2012], comparing them to some other bandit algorithms. In real world data CTS is the most effective.

==> PascalRename2.tex <==
\begin{table}[ht]
\centering
%%\tiny
\footnotesize
\caption{Results against PASCAL EvE Challenge 2006
\\(given as number of mistakes\(\times 10^{-3}\))}
\begin{tabular}{l r r r r}
\hline\hline
 & Random & DiscountedUCB & OCTS & OCTS2 \\
\hline
%%Where resMap should go%%
WeeklyCloseVariation & \(25.7\pm0.3\) & \(5.3\pm0.5\) & \(8.9\pm0.4\) & \(6.9\pm0.4\) \\
FrequentSwap & \(49.1\pm0.5\) & \(\mathbf{10.1\pm1.1}\) & \(27.9\pm2.4\) & \(12.5\pm1.3\) \\
Constant & \(20.0\pm0.1\) & \(5.5\pm0.5\) & \(\mathbf{0.6\pm0.1}\) & \(1.0\pm0.2\) \\
DailyVariation & \(57.2\pm0.3\) & \(7.9\pm0.9\) & \(17.1\pm0.3\) & \(6.6\pm0.3\) \\
LongGaussians & \(112.1\pm9.1\) & \(\mathbf{2.9\pm0.4}\) & \(4.4\pm0.4\) & \(3.4\pm0.5\) \\
WeeklyVariation & \(57.2\pm0.3\) & \(\mathbf{4.0\pm0.4}\) & \(8.2\pm0.3\) & \(5.3\pm0.5\) \\
%%Where resMap should go%%
\hline
Total & 321.3 & 35.7 & 67.2 & 35.8 \\
\hline
\end{tabular}
\\
%%\vspace{1cm}
\begin{tabular}{l r r r r}
\hline\hline
 & OCTSI & OCTSI2 & LOCTS & LOCTS2 \\
\hline
%%Where resMap should go%%
WeeklyCloseVariation & \(\mathbf{4.2\pm0.8}\) & \(6.2\pm0.4\) & \(8.9\pm0.4\) & \(9.0\pm0.3\) \\
FrequentSwap & \(13.7\pm1.6\) & \(15.1\pm1.7\) & \(28.2\pm2.7\) & \(14.8\pm1.2\) \\
Constant & \(3.2\pm0.4\) & \(2.0\pm0.3\) & \(0.3\pm0.2\) & \(0.8\pm0.2\) \\
DailyVariation & \(\mathbf{4.5\pm1.5}\) & \(4.9\pm0.5\) & \(17.6\pm0.3\) & \(16.0\pm0.3\) \\
LongGaussians & \(9.4\pm2.9\) & \(3.7\pm0.7\) & \(4.4\pm0.4\) & \(4.0\pm0.3\) \\
WeeklyVariation & \(4.7\pm1.7\) & \(5.4\pm0.5\) & \(8.5\pm0.3\) & \(8.4\pm0.3\) \\
%%Where resMap should go%%
\hline
Total & 39.6 & 37.4 & 67.9 & 53.1 \\
\hline
\end{tabular}
\\
%%\vspace{1cm}
\begin{tabular}{l r r r r}
\hline\hline
 & LOCTSI & LOCTSI2 & Adapt-EvE Meta & Adapt-EvE Meta $\rho$ \\
\hline
%%Where resMap should go%%
WeeklyCloseVariation & \(12.8\pm0.7\) & \(10.4\pm0.4\) & \(5.4\pm0.8\) & \(5.5\pm0.9\) \\
FrequentSwap & \(23.1\pm1.2\) & \(23.0\pm1.9\) & \(14.0\pm1.9\) & \(10.6\pm1.3\) \\
Constant & \(15.8\pm0.4\) & \(1.9\pm0.2\) & \(2.5\pm0.5\) & \(3.2\pm0.3\) \\
DailyVariation & \(15.1\pm1.0\) & \(24.2\pm0.3\) & \(6.2\pm0.7\) & \(6.1\pm0.7\) \\
LongGaussians & \(14.4\pm2.1\) & \(8.2\pm0.5\) & \(4.8\pm1.6\) & \(4.3\pm1.4\) \\
WeeklyVariation & \(12.1\pm1.1\) & \(11.7\pm0.4\) & \(4.8\pm0.8\) & \(5.1\pm0.9\) \\
%%Where resMap should go%%
\hline
Total & 93.2 & 79.3 & 37.7 & \textbf{34.7} \\
\hline
\end{tabular}
\vspace{1cm}
\label{tbl:Pascal2006}
\end{table}

